Q-MAML: Quantum Model-Agnostic Meta-Learning for Variational Quantum Algorithms

In the Noisy Intermediate-Scale Quantum (NISQ) era, using variational quantum algorithms (VQAs) to solve optimization problems has become a key application. However, these algorithms face significant challenges, such as choosing an effective initial set of parameters and the limited quantum processing time that restricts the number of optimization iterations. In this study, we introduce a new framework for optimizing parameterized quantum circuits (PQCs) that employs a classical optimizer, inspired by Model-Agnostic Meta-Learning (MAML) technique. This approach aim to achieve better parameter initialization that ensures fast convergence. Our framework features a classical neural network, called Learner}, which interacts with a PQC using the output of Learner as an initial parameter. During the pre-training phase, Learner is trained with a meta-objective based on the quantum circuit cost function. In the adaptation phase, the framework requires only a few PQC updates to converge to a more accurate value, while the learner remains unchanged. This method is highly adaptable and is effectively extended to various Hamiltonian optimization problems. We validate our approach through experiments, including distribution function mapping and optimization of the Heisenberg XYZ Hamiltonian. The result implies that the Learner successfully estimates initial parameters that generalize across the problem space, enabling fast adaptation.

==> 1_1_Approach.tex <==
We define task space of Q-MAML with diverse Hamiltonian, where each Hamiltonian is considered as a single problem to solve in VQE. We handle these probelms in \emph{Hamiltonian Task Space}. In this subsection, we illustrate the definition of \emph{Hamiltonian Task Space} with mathematical and empirical analysis. And we further specify the conditions required for good \emph{Hamiltonian Task Space}.
% \Revise{WRITE SMALL INTRO OF APPROACH} %Now we need to find the /emph{State} in the RL loop on the Quantum side. %Let's define this vector as the Representation Vector.
%\newline % Task Space의 조건 및 정의를 가져와서 힐베르트 공간의 완비성과 코시 수열의 수렴성 직교성, 무한 차원 등으로 논증할 예정
% In this perspective, the Hamiltonian can be thought of as acting as an environment.

%여기까지 개요인데 다듬어야 함
The Hamiltonian is a Hermitian operator that generates the time evolution of a quantum state. In Quantum Computing, the unitary operator $U$ is generated by Hamiltonian. 
\begin{equation}
    U(t)=exp(-\hat{H}t/\hbar)
\end{equation}
First, let's define the \emph{Task Space} of the Hamiltonian.
\begin{definition}[Hamiltonian]
The Hamiltonian operator H is a function defined in a Hilbert space $\mathcal{H}$ as follows:
\begin{equation}
    \hat{H}: \mathcal{H} \rightarrow \mathcal{H}.
\end{equation}
\end{definition}
% \Comment{What is Hamiltonian Task?}
% \Comment{i, n used duplicated times so I used k, m for this definition}
\begin{definition}[Hamiltonian Task Space]
    Let's denote the task space as $\mathcal{T}$. %If the task corresponds to a specific Hamiltonian \Comment{$\hat{H}_m$}, then task space can be defined as a set of Hamiltonians.
    Task space is defined as a set of Hamiltonian.
    \begin{equation}
        \mathcal{T} = \{\hat{H}_1,\hat{H}_2,...,\hat{H}_m\}.
    \end{equation}
\end{definition}
Considering that Hamiltonian serves as a fundamental link between the energy of a system and the quantum state, it is logical to construct task space with a set of Hamiltonian.
%Physically, Hamiltonian has a meaning that connects the energy and quantum state of each physical system, so it is natural to construct a task space with a set of Hamiltonian. \Comment{to jei see comment below}% it is natural 이라는게 물리적인 현상을 만드는게 헤밀토니안 이니까 뭔가 분류되는게? 모이는게 자연스럽다. 그래서 SET을 만든다 라고 녹여내고 싶음

\begin{definition}[Parameterized Hamiltonian Task Space]
When Hamiltonian $\hat{H}$ has representation vector $\phi$, we denote as follows:
%If appropriate $\phi$ can parameterize the Hamiltonian, and the space of its parameters is denoted by $\Phi$. Function $f$ define as follows:%\Revise{We can re-define task space $\mathcal{T}$ with parameterized Hamiltonian as follows:}
    \begin{equation}
    \begin{split}
    f: \Phi \rightarrow \mathcal{T}\\
    f(\phi_m)=\hat{H}_m
    \end{split}
    \end{equation}
\text{where} $\phi \in \Phi$.
\end{definition}

%A good parameterize is one where the distance between parameters is close~\cite{sun2022paco,hausknecht2015deep,ruckstiess2010exploring}, therefore \Revise{if we parameterize Hamiltonian well,} the corresponding Hamiltonian should be close as well. 
% \Comment{PaCo: Parameter-Compositional Multi-task Reinforcement Learning, Parameterized Action Spaces in Deep Reinforcement Learning --> Deep reinforcement learning in parameterized action space?, Exploring Parameter Space in Reinforcement Learning}
\begin{lemma}[The existence of a real-number parameter space]
There is at least one space $\Phi$ in the n-dimensional real-number vector space.
\begin{equation}
    \exists \Phi \subset \mathbf{R}^n
\end{equation}
\end{lemma}
\begin{proof}
    The existence can be demonstrated by considering the eigenvalues of the Hamiltonian as an example. It can be expressed as follows:
    \begin{equation}
        \hat{H} = \sum\limits_n E_i\ket{\psi_i}\bra{\psi_i}
    \end{equation}
    In quantum mechanics, the eigenvector of Hamiltonian forms a basis of Hilbert space. $E_i$ represents energy level and $\ket{\psi_i}$ represents its respect quantum state. Therefore, $E_i$ is a real number and $\ket{\psi_i}$ is a normalized orthogonal eigenvector. % In the eigenvalue problem of Hamiltonian, if the Hamiltonian $\hat{H}$ has n eigenvalues $E_n$, It is expressed as follows.
    % $\hat{H}$ is a self-adjoint operator. Thus, $E_n$ is real value. and $\ket{\psi_n}$ is a normalized orthogonal eigenvector. 
    In general, the Hamiltonian can be decomposed into the product of a unitary matrix $U$ and a diagonal matrix $D$:
    \begin{equation}
    \hat{H} = UDU^\dagger
    \label{eq:udu}
    \end{equation}
    where the diagonal values of $D$ is the eigenvalues of $\hat{H}$, which is real values. Therefore, if we take the diagonal of $D$ as $\phi$, we can define space $\Phi$ that is under real space.
    % \Revise{We define a diagonal vector as the representative vector of Task Space $\mathcal{T}$.}
    \begin{equation}
    \begin{split}
        \text{if}, \phi \equiv diag(D) \newline\\
        \text{then}, \Phi \subset \mathbf{R}^n
    \end{split}
    \label{eq:def}
    \end{equation}
    With~\refeq{def}, we successfully define the parameter space $\Phi$ that satisfies Lemma.
    % Then, We successfully define the parameter space $\Phi$.
\end{proof}
\renewcommand\qedsymbol{QED}
Through linear transformations, infinitely many distinct subspaces can be generated from a given vector space.

\begin{figure}[htbp]
    \centering
     \subfigure[Uniformly Sampled $J_U$]{\includegraphics[width=0.44\columnwidth]{figures/approach_uniform.png} \label{fig:xyz_app_grid}}
     \subfigure[Normally Sampled $J_N$]{\includegraphics[width=0.44\columnwidth]{figures/approach_normal.png} \label{fig:xyz_app_normal}}
    \caption{Relationship between distance in parameter space and task space}
    \label{fig:dimension}
\end{figure}


Using the eigenvalues of the Hamiltonian is an effective method for constructing a representation vector, as it allows us to infer the conditions for a good parameterization.
\begin{conjecture}[Conditions of good parameterizaion]
The good parameterization satisfies the following conditions:
    \begin{enumerate}
        \item Unique Representation\\
        $f$ \text{is injective with respect of} $\phi$
        \begin{equation}
            f(\phi_1) = f(\phi_2), \text{ then } \phi_1 = \phi_2
        \end{equation}
        \item Dimensionality \newline
        Minimize the number of parameters while retaining the model’s ability to adequately describe the Hamiltonian.
        \item Uniform continuity \newline
        Distance function in each space $d_{\Phi}$, $d_{\hat{H}}$ meet the following:
        \begin{equation}
        \begin{split}
            &\text{for every } \phi_1,\phi_2 \in \Phi\\
            &d_{\Phi}(\phi_1,\phi_2) < \sigma ,\text{then } d_{\hat{H}}(\hat{H}_1,\hat{H}_2) < \epsilon
        \end{split}
        \label{eq:conti}
        \end{equation}
    \end{enumerate}
\end{conjecture}
% \begin{example}
Conjectures 5.1 and 5.2 are well-founded, given the definitions of the task space and parameter space, which establish the relevant relationship and constraints. In contrast, the validity of Conjecture 5.3 is less supported by existing data or theoretical results. To show one example that follows Conjecture 5.3, we use a well-known Hamiltonian problem, the Heisenberg XYZ Hamiltonian. 

As we previously explained, Heisenberg XYZ Hamiltonian is defined via three parameters, $J_1$, $J_2$, and $J_3$ and can be obtained by calculating following equation:
% For example as the Heisenberg XYZ Hamiltonian \refeq{heisenberg}   that is defined via three parameters, $J_1$, $J_2$, and $J_3$ as following:
\begin{equation}
    \hat{H}_{XYZ} = - \sum\limits_{n=1}^{N-1} (J_1\sigma^1_n \sigma^1_{n+1} + J_2\sigma^2_n \sigma^2_{n+1} + J_3\sigma^3_n \sigma^3_{n+1})
    \label{eq:heisenberg_append}
\end{equation}
where $\sigma^1, \sigma^2, and \sigma^3$ represent the Pauli X, Y, and Z matrices, respectively.
If we define the distance in Hamiltonian space and parameter space as~\refeq{dist}, we can visualize the relationship between two spaces as in~\reffig{dimension}.
% In this analysis, The distance is defined as \eqref{eq:dist}, the relationship between the two distances can be depicted.
\begin{equation}
\begin{split}
    d_{\hat{H}}(f(\phi_i),f(\phi_j)) \equiv \braket{f(\phi_i)}{f(\phi_j)}\\
    d_{\phi}(\phi_i,\phi_j) \equiv \sum (\phi_i - \phi_j)
\end{split}
\label{eq:dist}
\end{equation}


Figure \ref{fig:xyz_app_grid} showing the parameterization method using $J$ meet the uniform continuity around the point $\hat{H}_{[1,1,1]}$. $J_U$ is sampled from the uniform distribution ($J_U = [J_1, J_2, J_3]$, $J_i \sim \mathcal{U}(-3,5)$). 
Figure \ref{fig:xyz_app_normal} shows that two spaces are linearly correlated around the point $\hat{H}_{[1,1,1]}$. $J_N$ sampled from normal distribution ($J_N = [J_1, J_2, J_3]$, $J_i\sim \mathcal{N}(1,1)$).
According to the results, a good parameterization should satisfy uniform continuity. Specifically, a parameterization based on eigenvectors will be differentiable if and only if the Hamiltonian is differentiable~\cite{smale1967differentiable}.

% \end{example}
% \Revise{We show that the distance between the task space (Hamiltonian) and parameter space uniform continuity is linearly correlated (see Figure \ref{fig:dimension}). Around a point $\hat{H}_{[1,1,1]}$.}
% \begin{figure}[t]
%  \centering
%  \subfigure[Training Dynamics]{\includegraphics[width=0.4\columnwidth]{figures/epoch_accuracy_compare_230516_ver2.pdf} \label{fig:epoch-dynamics}}\hspace{3mm}
%  \subfigure[Accuracy Improvement]{\includegraphics[width=0.42\columnwidth]{figures/accuracy_accimp_selection_230517_ver1.pdf} \label{fig:improvement}}
% \vspace{-2mm}
%  \caption{Training dynamics for the most effective case of the target task 14 using the backbone task of 4 and accuracy improvement with respect to the smoothed accuracy of \emph{w/o Backbone}%before knowledge federation
%  . The smoothed accuracy refers to the averaged accuracy accumulated for a subset of tasks selected from those with lower accuracy. For example, the second value in the graph represents the average accuracy of the two tasks with the lowest performance, while the last value is the average across all tasks}
%  \vspace{-5mm}
%  \label{fig:backbone-selection}
% \end{figure}


% 증명 1
% 헤밀토니안을 매개변수화 할 때, 적절한 매개변수가 유클리드 공간에 존재하는가?
% 이는 H(θ)가 θ에 대해 미분 가능하거나, 연속적으로 변화할 수 있음을 의미함.
% 매개변수 θ에 대해 H(θ)가 미분 가능하면, 그 공간은 유클리드 공간으로 매개변수화 될 수 있다. 그리고 연속적으로 의존한다면, 그 매개변수 공간은 R^n인 유클리드 공간으로 생각할 수 있다.
% 의존성은 대부분의 물리적 기저에서 매개 변수가 유클리드 공간에서의 물리적 의미가 있음. 따라서 헤밀토니안이 θ에 의존적인것은 자연스러움.
% 미분가능성 헤밀토니안은 미분됨. 근데 매개변수에 대해 미분됨? 존재성의 증명
% 매개변수가 eigen value라면, 

% 증명 2
% 힐베르트 공간은 Task Space로 적절한가?



% We use the Heisenberg XYZ Hamiltonian for the experiment. which is defined with three variables.
% Each variable was sampled from a normalized distribution with sigma equal to 1 centered on [1,1,1].
% \begin{equation}
%     J = [J_1, J_2, J_3], J_i \sim \mathcal{N}(1,1)
% \end{equation}
% and the trend line was plotted.
% We found that the distance between two spaces is linearly correlated.
%Therefore, \Revise{it can be experimental evidence} that it is reasonable to parameterize the Hamiltonian by a real number vector.
% \Comment{Check following paragraph}

% For backpropagation, we need to calculate the gradient of the Learner using the cost function. Applying chine-rule, \Revise{the backpropagation of the Learner can be described as follows: }%It can describe eq.
% \begin{equation}
%     \frac{dl_T}{d\phi} = \frac{dl_T}{dU} \frac{dU}{d\theta} \frac{d\theta}{dW} \frac{dW}{d\phi}.
% \end{equation}
% $\frac{dU}{d cost}$ Most of the cost functions are differentiable. $\frac{dU}{d\theta}$ PQC is generally differentiable, although this is depending on the circuit architecture. $\frac{dW}{d\theta}$,  Neural Networks are differentiable.
% Then, we can obtain $\frac{dW}{d\phi}$.

